Reasoning Through Execution: Unifying Process and Outcome Rewards for Code Generation

Large Language Models excel at code generation yet struggle with complex programming tasks that demand sophisticated reasoning. To bridge this gap, traditional process supervision relies on learned reward models requiring costly training data and suffering from reward misalignment, while outcome supervision fails for complex tasks needing coordinated intermediate steps. We introduce Outcome Refining Process Supervision, which unifies process and outcome supervision by leveraging executable verification: a tree-structured search framework generates strategic alternatives, profiles execution metrics, and scores candidates via self-critique mechanisms that integrate runtime feedback with reasoning. Experiments across 5 models and 3 benchmarks show consistent gains, with 26.9% higher correctness and 42.2% improved code efficiency. The results demonstrate that ORPS enables LLMs to overcome local optima in code generation, suggesting a promising direction for combining verifiable outcomes with structured reasoning to tackle complex challenges. We open-source at: https://github.com/zhuohaoyu/ORPS

==> sec6-limitations.tex <==
\section{Limitations}
While \ourmethod~ demonstrates significant advancements in code generation, it has notable limitations. First, its reliance on execution outcomes as primary feedback restricts its applicability to tasks where execution is feasible and well-defined. Ambiguous problem descriptions or creative tasks beyond executable code can hinder the framework’s performance. Additionally, this reliance may lead to a bias toward solutions optimizing immediate execution success, potentially overlooking broader algorithmic considerations.

The tree-structured beam search also introduces significant computational overhead, requiring substantial memory and processing power. While scalable with increased resources, this approach may be impractical for real-time or resource-constrained applications, limiting its utility in some environments.

Finally, the quality of \ourmethod ~depends heavily on the underlying language model. If the model lacks domain knowledge or reasoning ability, it may generate incoherent reasoning chains or fail to explore promising solutions effectively, especially when feedback mechanisms rely solely on execution outcomes without additional validation.

==> sec7-ethical.tex <==
\section{Ethical Considerations}
While \ourmethod~advances code generation capabilities, we acknowledge important ethical considerations. Like all LLM-based systems, our framework inherits potential biases from the underlying models. However, our execution-guided approach provides an advantage: concrete verification helps detect and mitigate certain failure modes through objective testing. The framework's ability to explore multiple solution paths also reduces the risk of being stuck with problematic implementations.

We emphasize that \ourmethod~is designed as a development aid rather than a replacement for human programmers. The execution feedback and reasoning traces make the code generation process more transparent and auditable. We encourage using this framework in conjunction with established software development practices, including code review and testing, particularly for applications in sensitive domains.
